Fluid-solid Floquet stability analysis of self-propelled heaving foils

We investigate the role of linear mechanisms in the emergence of nonlinear horizontal self-propelled states of a heaving foil in a quiescent fluid. Two states are analyzed: a periodic state of unidirectional motion and a quasi-periodic state of slow back & forth motion around a mean horizontal position. The states emergence is explained through a fluid-solid Floquet stability analysis of the non-propulsive symmetric base solution. Unlike a purely-hydrodynamic analysis, our analysis accurately determine the locomotion states onset. An unstable synchronous mode is found when the unidirectional propulsive solution is observed. The obtained mode has a propulsive character, featuring a mean horizontal velocity and an asymmetric flow that generates a horizontal force accelerating the foil. An unstable asynchronous mode, also featuring flow asymmetry and a non-zero velocity, is found when the back & forth state is observed. Its associated complex multiplier introduces a slow modulation of the flapping period, agreeing with the quasi-periodic nature of the back & forth regime. The temporal evolution of this perturbation shows how the horizontal force exerted by the flow is alternatively propulsive or resistive over a slow period. For both modes, an analysis of the velocity and force perturbation time-averaged over the flapping period is used to establish physical instability criteria. The behaviour for large solid-to-fluid density ratio of the modes is thus analyzed. The asynchronous fluid-solid mode converges towards the purely-hydrodynamic one, whereas the synchronous mode becomes marginally unstable in our analysis not converging to the purely-hydrodynamic analysis where it is never destabilised.

==> macros.tex <==
%% WRITING

\newcommand{\comment}[1]{{\color{magenta}{[#1]}}}
\usepackage{caption} 
\newcommand{\ccaption}[2]{\caption{\small{\textit{\textbf{#1.} #2 }}}}

\newcommand\inv[1]{#1\raisebox{1.15ex}{$\scriptscriptstyle-\!1$}}	% for the inverse of matrices

\newcommand*{\mathcolor}{}
\def\mathcolor#1#{\mathcoloraux{#1}}
\newcommand*{\mathcoloraux}[3]{%
  \protect\leavevmode
  \begingroup
    \color#1{#2}#3%
  \endgroup
}

\newcommand{\FreeFem}{\texttt{Freefem++}}
\newcommand{\Arpack}{\texttt{ARPACK }}

%% OPERATORS (GENERAL)

\newcommand{\CConj}{\mbox{c.c.}}					% Complex conjugate
\newcommand{\ve}[1]{\mathbf{#1}}					% Vector
\newcommand{\te}[1]{\boldsymbol{\operatorname{#1}}}			% Tensor/matrix
\newcommand{\tf}[1]{\check{#1}}						% Test-function
\newcommand{\dpart}[2]{\frac{\partial #1}{\partial #2}}			% partial derivative
\newcommand{\ddroit}[2]{\frac{\diff #1}{\diff #2}}			% straight derivative
\newcommand{\dt}[1]{\frac{\partial #1}{\partial t}}			% t partial derivative
\newcommand{\dx}[1]{\frac{\partial #1}{\partial x}}			% x partial derivative
\newcommand{\dy}[1]{\frac{\partial #1}{\partial y}}			% y partial derivative
\newcommand{\dxx}[1]{\frac{\partial^2 #1}{\partial x^2}}		% xx partial derivative
\newcommand{\dyy}[1]{\frac{\partial^2 #1}{\partial y^2}}		% yy partial derivative
\newcommand{\dxy}[1]{\frac{\partial^2 #1}{\partial x \partial y}}	% xy partial derivative
\newcommand{\dyx}[1]{\frac{\partial^2 #1}{\partial y \partial x}}	% yx partial derivative
\newcommand{\mat}[1]{\begin{bmatrix} #1 \end{bmatrix}}			% Matrix
\newcommand{\conj}[1]{{#1}^{\star}}					% Conjugate
\newcommand{\adj}[1]{{#1}^{\dagger}}					% Conjugate
\newcommand{\ldeux}[1]{\left\| #1 \right\|_2}				% 2-norm
\newcommand{\pscal}[2]{\langle #1 , #2 \rangle}				% Scalar product
\newcommand{\mean}[1]{\overline{#1}}					% Mean value
\newcommand{\meanB}[1]{\overline{#1}_\text{B}}				% Filtred value
\newcommand{\diff}{\mathrm{d}}						% Differenciation
\newcommand{\im}{\mathbf{i}}						% imaginary number
\newcommand{\trans}{\operatorname{T}}					% Transpose
\newcommand{\transconj}{\operatorname{H}}				% Transpose-conjugate
\newcommand{\Id}{\operatorname{Id}}					% Identity
\newcommand{\real}{\mathfrak{Re}}					% Real part
\newcommand{\imag}{\mathfrak{Im}}					% Imaginary part
\newcommand{\indI}{\text{\tiny{I}}}					% Indice for imaginary parts
\newcommand{\indR}{\text{\tiny{R}}}					% Indice for real parts
\newcommand{\nablaE}{\nabla_\text{\tiny{E}}}				% Nabla operator in Euler coordinates
\newcommand{\opN}{\mathcal{N}} 						% N.S. Operator : (u.grad)u
\newcommand{\opC}{\mathcal{C}}						% C(a,b) = (a.grad)b+(b.grad)a
\newcommand{\opL}{\mathcal{L}}						% L(u,p) = grad(p)-1/Re*lap(u)
\newcommand{\opLc}{\mathcal{L}^\text{c}}				% L(u,p) = grad(p)-1/Re*lap(u) at the criticity
\newcommand{\opB}{\mathcal{B}}
\newcommand{\opF}{\mathcal{F}}

%% VECTORS

\newcommand{\ns}{\ve{n}}			% Solid outward normal
\newcommand{\ey}{\mathbf{e_y}}
\newcommand{\ex}{\mathbf{e_x}}
\newcommand{\ez}{\mathbf{e_z}}
\newcommand{\et}{\mathbf{e_t}}
\newcommand{\en}{\mathbf{e_n}}


\newcommand{\Rey}{\mathcal{R}e}
\newcommand{\Rec}{\Rey_{c}}
\newcommand{\Recp}{\Rey_{c,p}}
\newcommand{\Cd}{\mathcal{C}_D}
\newcommand{\Cl}{\mathcal{C}_L}
\newcommand{\Fd}{\mathcal{F}_D}
\newcommand{\Fl}{\mathcal{F}_L}

\newcommand{\uu}{\mathbf{u}}
\newcommand{\x}{\mathbf{x}}

%% Base fields
\newcommand{\uub}{\mathbf{u}_b}
\newcommand{\pb}{p_b}
\newcommand{\qb}{{\ve{q}_b}}
\newcommand{\ub}{u_b}
\newcommand{\vb}{v_b}

\newcommand{\I}{\mathbf{Id}}


\newcommand{\Grad}[1]{\nabla #1}
\newcommand{\Div}[1]{\nabla \cdot #1}
\newcommand{\Lap}[1]{\nabla^2 #1}

% Functionnal spaces
\newcommand{\Vens}{\mathcal{V}}
\newcommand{\Vf}{\mathcal{V}^{\text{f}}}
\newcommand{\Vs}{\mathcal{V}^\text{s}}
\newcommand{\Hun}{\mathcal{H}^1}
\newcommand{\Ldeux}{\mathcal{L}^2}
\newcommand{\Vh}{\mathcal{V}_h}
\newcommand{\Qh}{\mathcal{Q}_h}

% Newton Method & Stab Ana
\newcommand{\rNS}{\mathcal{R}}
\newcommand{\JacNS}{{\mathcal{J}_\text{b}}}
\newcommand{\puu}{{\mathbf{u}'}}
\newcommand{\pp}{{p'}}
\newcommand{\puuh}{{\hat{\mathbf{u}}}}
\newcommand{\pph}{{\hat{p}}}


\newcommand{\A}{{A}}
\newcommand{\W}{{W}}
\newcommand{\Aal}{{A_{\gamma}}}
\newcommand{\Apal}{{\hat{A}_{\gamma}}}
\newcommand{\Aununpmal}{{\hat{A}_{11}}}
\newcommand{\Adeuxdeuxpmal}{{\hat{A}_{22}}}
\newcommand{\B}{{B}}
\newcommand{\PAL}{{\mathcal{P}_{AL}}}
\newcommand{\PMAL}{{\mathcal{P}_{MAL}}}
\newcommand{\SCal}{{S}}
\newcommand{\SCpal}{{\hat{S}}}
\newcommand{\Aeig}{{\mathcal{J}}}
\newcommand{\Beig}{{\mathcal{M}}}

% Miscellaneous
\newcommand{\test}[1]{\check{#1}}
\newcommand{\Zm}{\mathbf{0}}
\newcommand{\Unm}{\mathbf{1}}
\newcommand{\nArnoldi}{n_{Arnoldi}}
\newcommand{\nrecycle}{n_{recycle}}

% -------------------
